When Bioprocess Engineering Meets Machine Learning: A Survey from the Perspective of Automated Bioprocess Development

Machine learning (ML) is becoming increasingly crucial in many fields of engineering but has not yet played out its full potential in bioprocess engineering. While experimentation has been accelerated by increasing levels of lab automation, experimental planning and data modeling are still largerly depend on human intervention. ML can be seen as a set of tools that contribute to the automation of the whole experimental cycle, including model building and practical planning, thus allowing human experts to focus on the more demanding and overarching cognitive tasks. First, probabilistic programming is used for the autonomous building of predictive models. Second, machine learning automatically assesses alternative decisions by planning experiments to test hypotheses and conducting investigations to gather informative data that focus on model selection based on the uncertainty of model predictions. This review provides a comprehensive overview of ML-based automation in bioprocess development. On the one hand, the biotech and bioengineering community should be aware of the potential and, most importantly, the limitation of existing ML solutions for their application in biotechnology and biopharma. On the other hand, it is essential to identify the missing links to enable the easy implementation of ML and Artificial Intelligence (AI) tools in valuable solutions for the bio-community.

==> tex/Impact.tex <==
%\section{Impact}

...In the next 5 years: making bioprocess systems research FAIR \cite{grandcolas2019rise,jacobsen2020fair} - Findable, Accessible, Interoperable, and Re-usable...






==> tex/Introduction.tex <==
%\section{Introduction}

Computational methods have been widely used in all systems engineering fields (e.g. electrical, chemical, aeronautics) to achieve a deep understanding of the process and a holistic optimization of it. 
Bioprocess engineering has been an exception though, with a significantly higher degree of empiric procedures, experts based decisions, and strongly segmented design strategies. 
The high complexity of living organisms with thousands of intracellular biochemical reactions and uncomprehended changes in its metabolic activity combined with the difficulties to obtain trustworthy observations makes it very difficult to build the mathematical models that are so crucial for the application of control and optimization methods. 
Furthermore, the large number of existing and emerging microorganisms together with the rapid mutation and screening methods developed oblige research and development to deal with new systems on a daily basis. 
%Added to these, the incredibly large profit margins compared to bulk chemical manufacturing (100 $/gallon vs 10 mio $ per gram) kept the pressure to maximize the profits low and focused on quality and process robustness instead up to the last decade.

This tendency has nevertheless seen drastic changes in recent years, the main drivers being i) the rapid development of Process Analytical Tools (PAT) \cite{kansakoski2006process,glassey2011process,simon2015assessment} that allow a deeper understanding of the processes, ii) the technological advances of High Throughput (HT) Liquid Handling Stations (LHS) \cite{diederich2017high,barz2018adaptive,hans2018automated} that generate large amounts of experimental data, and also iii) the significant increase in market pressure through expiration of patents, new analoga, as well as the society pressure to shift to environmental friendly production chains. 
Not only are biotechnology and biopharma industries investing huge amounts of resources to "digitalize" development and production \cite{scheper2020digitalization,narayanan2020bioprocessing,chen2020digital}, but also science and research have shown a clear interest on data science, statistics, machine learning, artificial intelligence, and model-based process design, control, and optimization methods for biopharma, biotechnology and bioprocesses.

Yet, there is an important link missing towards a truly bioprocess systems engineering procedure \cite{koutinas2012bioprocess}: the conversion of automated experimental tasks and data (e.g. cultivation, sampling, analytics) into knowledge expressed in mathematical expressions. 
And the large amounts of heterogeneous low quality data makes manual treatment and model development mostly impossible. 
Hence, a truly bioprocess systems engineering approach is only possible through the use and adaptation of existing machine intelligence methods. 
These tools need to be tailored to the challenges of bioprocesses aiming to transform HT experimental data into information, information into knowledge catched in mathematical mdodels, and to use this knowledge to understand, control, and optimize bioprocesses, biopharma, and biomanufacturing as a whole. 

#####

Modern biolabs have automatized and parallelized a large number of tasks, such that up to thousands of experiments can run in a day. These robotic experimental facilities equipped with Liquid Handling Stations (LHS), parallel cultivation systems, and High Throughput analytical devices are capable of generating very large data in short time. The focus in the past decade was set on hardware development and integration with mostly basic data management tools and rarely having advanced control and experimental design tools. In other words, despite of the fast generation of data, the current bottle-neck - that is automated data treatment, curation, and model building - remains unsolved. Currently, we have not been able to trigger the fruitful symbiosis that is expected between i. robots that can perform thousands of complex tasks but are waiting for humans to design the experiments, ii. Active Learning (AL) algorithms that are waiting for humans to perform the designed experiments, and iii. ML tools that are waiting for humans to treat and deliver the data in a machine readable form.

This reviews follows two important aims. On the one hand, the biotech and bioengineering community should be aware of the potential, and most importantly, of the limitation of existing ML solutions for its application in biotechnology and biopharma. On the other hand, it is essential to identify the missing links to enable the easy implementation of ML and AL solution in useful solutions for the bio-community.

#####

In the wake of climate change, many industries are turning to biotechnology to find sustainable solutions. The importance of biotechnological processes in pharmaceuticals is reflected in the growth figures for biopharmaceuticals (up 14 \% to 30.8 \% market share from 2020 to 2021)\cite{lucke_medizinische_2021}. 
This trend is currently strongly inhibited by the long development time of biotechnological processes.
In bioprocess engineering, bioprocesses are developed and optimized. Scalable process parameters enable a rapid transition from laboratory to production scale. 
Usually, different microorganisms or cells are tested to produce an industrial relevant product, I.e., a pharmaceutical substance. The transfer of results from small to large scale represents a central challenge and is very time-consuming. Miniaturized and versatile multi-bioreactor systems combined with LHS have the potential to make a significant contribution to the rapid and successful upscaling of biotechnological processes from laboratory scale to industrial production facilities.
Using multi-parallel minibioreactor systems combined with machine learning, the development time of bioprocesses is shortened and enables faster market entry.

\hl{Bioprocess engineering is...


Tranditional approaches of bioprocess engineering are...



The main challanges in improving tranditional approach of bioprocess engineering are...
}



Control of a bioreactor is a major issue in bioprocess. Especially in the fed-batch cultivation, both overfeeding and underfeeding yield inferior results on the cell growth and product formation \citep{lee1999control}. The key to the reliable control method is to act against high level of uncertainties originating from low amount and quality data and significant variabilities in the process variables and cell metabolic. Given these complexities, ``closed-loop'' is an important feature, reflecting the most recent information (measurements) and adapting the control strategy. While basic feedback controllers such as PID controller have been widely applied, incorporating biological model and optimization become increasingly important to account for economic objectives and process constraints. This is typically coupled with filtering or parameter estimation methods \citep{lucia2017rapid, elsheikh2021comparative}.  

Fed-batch bioprocess control problems are in general classified into two; high-level economic optimization and low-level tracking control \citep{yoo2021reinforcement}. In the high-level optimization, an economic objective which is related to the final product quality requirements or experimental design is optimized by the feed rates and other manipulated variables. Because controller has to handle the nonlinearity caused by the wide operating region along the long-term operation, model-based optimal control methods have been preferred. Model predictive control (MPC) has been one of the most popular approaches for the high-level optimization \citep{ashoori2009optimal, raftery2017economic}. Due to the high computational complexity of the optimization, open-loop method is often taken \citep{lee1999control, schorsch2019optimal}. Recent studies recognize the importance of model adaptation (less frequent than that of the low-level), therefore optimal state or parameter estimators such as Kalman filter \citep{markana2018multi, hong2021mechanistic} or MHE \citep{abdollahi2012lipid, del2016model} are jointly used with the MPC. Low-level control, in contrast, is responsible for the online implementation of the optimal trajectory computed at the high-level counterpart. The problem is typically formulated as a tracking control, while rejecting real-time disturbances. Because online implementation requires the decision to be updated more frequently, controllers should have lower complexity. For controlling actuator-level process variables such as temperature, pH, or stirring rate, PID controller \citep{birol2002modular, pachauri2017two} or fuzzy controller \citep{cosenza2012nonlinear} are widely used. MPC that considers short-term prediction are implemented, as path constraints are also critical in the low-level tracking control \citep{ramaswamy2005control, tebbani2008open}.

Several studies have incorporated model-based methods for HT experiments of fed-batch mini-bioreactors. The main challenges are the i) addressing impulsive control systems due to bolus-feeding for miniaturized system, ii) ill-conditioned parameter estimation, and iii) parallel control. In the work of \citep{cruz2017online, barz2018adaptive, kim2021oed}, optimal experimental design problems were studied to maximize the information content for effective identification of the model. MPC and MHE aiming at maximizing cell growth were implemented to an in silico system \citep{kim2022model} and validated through the experiment \citep{krausch2022high}.

With the increasing applications of model-based methods to the bioprocesses, a critical challenge arises: The performance depends strongly on the quality of the mechanistic model. Mechanistic model cannot solely solve this issue. The latest trend clearly shows that we need the machine learning techniques that allow for the efficient utilization of data. According to \citep{venkatasubramanian2019promise}, the machine learning was not as extensively used to the bio-chemical processes as it had been anticipated compared to the big-data domains such as vision, natural language processing, and speech recognition. Bioprocess modeling problems are extremely challenging and the bioprocess. Moreover, experimental data is not aggregated across the laboratory, expensive to generate, and has low reproducibility.


 ML for better forecasting, RL for not even using the model. \citep{venkatasubramanian2019promise}


Machine learning is a viable and effective solution to these mentioned problems. 
Over the past few decades, bioprocessing has seen a significant shift from manual modeling to data-driven modeling, e.g., applying machine learning, partly due to the large amount of accumulated data \cite{mowbray2021machine,lawson2021machine,scheper2020digitalization}. 
It is an important premise for integrating machine learning models into well-informed bio-data, creating great potential for discovering advances in the field of bioprocessing \cite{narayanan2020bioprocessing,neubauer2017bioprocess,neubauer2020potential}. 
Machine learning itself is also enhanced through a wide range of research in mathematical foundations, modeling, and computational hardware. 
Besides, machine learning also makes itself easier to use for experts in other fields. 
They do not need to spend time understanding the principles for each model, but can conveniently call the model upon specific data type. 
This fascinating feature has attracted many bioengineering experts and encouraged the application of machine learning to biological processes that are considered among the most complex in the world. 
In fact, machine learning has proven its effectiveness in many areas of biology: 3D structure of proteins \cite{wei2019protein,jumper2021highly}, up-downstream processes \cite{kaspersetz2022automated,schonberger2018deep,haque2016artificial,walther2022smart}, bioprocessing for chemical and biologic product manufacturing \cite{scheper2020digitalization,petsagkourakis2020reinforcement}, enzymes and cell growth \cite{mazurenko2019machine,heckmann2018machine,tan2019survey}, cell culture expression systems \cite{barz2022characterization,borisov2017individual,ashraf2021applying}, and many others. 
However, it should be understood that machine learning is not a miracle that can solve all existing problems, not just taking the state-of-the-art machine learning models and applying on certain biological data. 
Machine learning is just one part of the whole biological process which includes the problem description, the data it can collect, what machine learning can accomplish, the output of the machine learning model to be used further. 
In the bioprocessing process, biological knowledge is essentially required to select the optimal hyperparameters for the machine learning model that help boost its peak performance. 
Note that a machine learning model focuses on making predictions based on data. 
In the meantime, bioprocessing experts must identify the desired inputs and outputs of the machine learning model, the value science around integrating machine learning into biological processes \cite{volk2020biosystems}. 
What does machine learning perform well, but the intrinsic problems of bioprocessing hinder the usability of the model? 
Why are biological experimental procedures so difficult to replicate elsewhere? 
In fact, choosing a machine learning algorithm for a bioprocessing engineering problem is much more complex. 
The selection of the most efficient algorithm is based on many factors, including the transformation from a bioprocessing engineering problem into machine learning tasks, the quantity and quality of the data collected, the availability of the data labels, the type of problem being solved (regression, classification, forecasting, etc.), the degree of integration of the outputs into the biological process, the required overall accuracy and performance, prior bioprocessing knowledge to control the hyperparameters tuning \cite{niazi2017fundamentals,neubauer2017continuous}, and the hardware system investment to ensure processing capacity. 
With a complex problem involving the multi-dimentionality of many different fields, technical constraints, and experts in each of those fields, the optimal choice of machine learning models for each bioproblem is not trivial task. 
This constitutes a significant barrier for bio-experts desiring applying the latest machine learning methods in their field.


In this work, we review the existing applications of machine learning and artificial intelligence in bioprocess engineering. We mostly focus on the existing tools that, in our opinion, have not been considered yet despite having a great potential to solve critical challenges in bioprocess development and engineering.







==> tex/Motivations.tex <==
%\section{Motivations}

The trend of integrating machine learning and artificial intelligence into bioprocessing engineering process is inevitable, clearly shown by the research over the past decades \cite{oliveira2019biotechnology,aransiola2021challenges,wackett2022future}. 
The benefits of both fields, although different, can be combined: the predictive power of machine learning models increases as more data is available, and bioprocessing becomes more efficient when integrates multiple machine learning models. 
In this combination, the machine learning approaches focus on enhancing predictive capabilities, while the bioprocessing engineers concentrate on the scientific merits of the system as a whole, incorporating an understanding of the biophysics processing. 
Understanding this combination is crucial in the development of bioprocess techniques because it leads to knowledge that can actually be leveraged to predict the outputs of a biological system.

Perhaps the most difficult challenge for this combination is that biological data sources are diverse, distributed, and multi-structured. 
It results in highly heterogeneous bioprocessing data and requires a great deal of data preprocessing techniques to be used before applying any machine learning algorithms. 
Secondly, the biological data's copyright is also a barrier to future collaborative development.
Several data sources require an access fee or be released upon a reasonable request, see some examples listed in Table \ref{tab:app-ml-bio-eng}. 
Thirdly, data collection methods in bioengineering are highly dynamic since many biological process parameters are collected online as continuous measurements and are highly dependent on the quality of measurement system, quality of experimental system, chemical quality, water source, frequency of measurements (e.g., temperature, optical density, pH, oxygen, glucose, oxygen uptake rate, stirring spped). 
The progress is also up to the technician as he or she conducts the scheduling. 
In addition to online parameters, bioengineering experiments can include many offline measurements (e.g., chemical concentration, product concentration, substrate consumption rate). 
There are also influencing factors such as the latency of the robotic system controlling the sensors, the periodic sizing of the experimental equipment, the cumulative error of the physical systems. 
As a result of the factors just listed, the data collected is highly heterogeneous, requires manual intervention by technicians, and greatly limits efforts to construct standard datasets. 
If the data cleaning and normalization process is not good and standardized, the metadata (information that describes the process of performing any bioengineering experiment) is in an even worse state. 
Without careful investment in this piece of data infrastructure, there is little hope for the disruptive impact of machine learning in bioprocessing engineering. 
This prevents the effectiveness of machine learning models.

In contrast, bioprocessing techniques with many interesting problems can also become an inspiration for machine learning algorithms. 
From data source perspective, bioprocessing engineering data is also a form of data that machine learning engineers have worked through, e.g., images, sounds, text, time series. 
Therefore, it is not unreasonable to assume that bioprocessing techniques can be an inspiration for the application and development of better models. 
A complete understanding of bioprocessing, how biological experiments operate, the different principles of test description, high-throughput analysis, and synthetic biology, can provide detailed valuable information for the proposal and development of new machine learning methods. 
The authors believe that using machine learning to enhance the bioprocessing's automation with less manual intervention can significantly increase reproducibility. 
Another, often overlooked, non-technical obstacle that limits the integration of machine learning and bioprocessing involves a process challenge with very little interference. 
Therefore, communication between the two groups is often complicated by these differences. 
This creates problems in aligning goals and project management interests. 
However, communication is necessary, even machine learning researchers cannot keep up with the literature of their field, there is no way they have to understand the full details of bioprocess domain, and vice versa.
The authors argue that only through an interdisciplinary effort can the best of both fields be combined to create something greater than the sum of its disjointed parts.







==> tex/Summary.tex <==
%\section{Summary}

In this discussion, we provide a thorough and comprehensive survey of existing works in bioMoCoML.
We summarize...







==> tex/motivations-new.tex <==
Automation of the model building cycle aims to facilitate and transform the decision-making context of bioprocess engineers as well as of biotechnology experts and scientists, not to replace them. Some aspects of model building are more difficult to automate, not only because of technological challenges, but because they involve open-ended questions and context-dependent tasks that require human intervention. Perhaps the most difficult challenge to model building automation is that data sources in the development pipeline are diverse, distributed, and multi-structured. Moreover, not only available data is highly heterogeneous, but also may be no informative regarding the purpose of the model for a given stage. This contrasts sharply with the common assumption that sufficient amounts of high-quality data are available for model building. Data collection methods for bioprocess development are descriptive of an inherently dynamic behavior since many process parameters are gathered online as continuous measurements are available and are highly dependent on the quality of sensor devices, standard operating procedures, material and methods used, frequency of measurements (e.g., temperature, optical density, pH, oxygen, glucose, oxygen uptake rate, stirring speed), analytical sample processing, calibration parameters, etc. Then, the optimal design of experiments for gathering informative must be an integral part of the model building cycle. As a result, model building at the different stages of bioprocess development will comprise of automated procedures for actively seeking or generating highly informative data regarding the objective and type of decisions that must be taken in each stage in Fig. 1.

Faced with the choice from a large set of machine learning algorithms and an even larger space of hyperparameter settings, even experts often must resort to costly experimentation in time and money to determine what combination works best for a given problem. Hence, automated model building approaches must be necessarily end-to-end, and thereby not only spares non-experts the time and effort of extensive, often onerous trial-and-error experimentation, but also enables bioprocess engineers to obtain substantially better performance with less data and faster than otherwise possible without automation. In some applications of reinforcement learning to control and optimization, close-loop experimentation must be part and parcel of the model building cycle which makes automation even more important. Hyperparameters in this case drive learning and define which data is actually gathering in the learning curve. Without a meta-learning level in model building the initial setting of hyper-parameter can easily prevent learning a predictive model that can make a real difference with no using a model at all for taking decisions.
The use of machine learning for model building automation can be seen as a way of introducing another level of abstraction to focus expert humans in the most cognitive tasks of bioprocess development. First, there is the use of probabilistic programming for autonomous building of predictive models. Second, machine learning automatically assess alternative decisions by first planning experiments to test hypothesis and then carrying out experiments to gather informative data that focus on models selection based on the uncertainty of model predictions. Therefore, machine learning methods can be seen as meta-algorithms for model building tasks, and hence automate both data generation and hypothesis testing. Finally, automated model building makes use of algorithms that select and configure machine learning algorithms—that is, of meta-meta-algorithms that can be understood as Bayesian machine experimenters that generate new data to transform a priori knowledge into rational decisions that further bioprocess development.





==> tex/neuralode.tex <==
Since their inception in the 17th century, differential equations have become an indispensable tool in the sciences for modeling continuous time dynamical systems.

In 2018, Che et al. first introduced a machine learning framework that represents the vector field of an ordinary differential equation by an artificial neural network and allows learning the system dynamics from observational data. Since then, there has been a bloom of ODE based machine learning models, ranging from time-series forecasting models over ... to models that discover conservation laws.
